InferSpark: Statistical Inference at Scale

The Apache Spark stack has enabled fast large-scale data processing. Despite a rich library of statistical models and inference algorithms, it does not give domain users the ability to develop their own models. The emergence of probabilistic programming languages has showed the promise of developing sophisticated probabilistic models in a succinct and programmatic way. These frameworks have the potential of automatically generating inference algorithms for the user defined models and answering various statistical queries about the model. It is a perfect time to unite these two great directions to produce a programmable big data analysis framework. We thus propose, InferSpark, a probabilistic programming framework on top of Apache Spark. Efficient statistical inference can be easily implemented on this framework and inference process can leverage the distributed main memory processing power of Spark. This framework makes statistical inference on big data possible and speed up the penetration of probabilistic programming into the data engineering domain.

==> inference.tex <==
\subsection{Inference algorithms}
\label{sec:inference}
\begin{itemize}
\item Variation message passing
\item Gibbs sampling
\end{itemize}

\KZ{And how to switch between the two.}


==> motivate.tex <==
\section{Motivating Examples}
\label{sec:motivate}

\subsection{Latent Dirichlet Allocation}

Latent Dirichlet Allocation (LDA) is widely used for topic modelling. In LDA,
each word in the documents has a corresponding latent topic and the word is
viewed as a random sample from the categorical distribution associated with
the latent topic. The topics in a document conform to a document-specific
categorical distribution. Dirichlet priors are used on the topic-word and
document-topic categorical distribution. 

The LDA model is in the exponential family and each node has conjugate priors.
As a result, the variational message passing algorithm can be applied
automatically to the inference problem of LDA, which is equivalent to the
original algorithm proposed in \cite{blei2003latent}. The alternate inference
technique involves creating a collapsed Gibbs Sampler
\cite{griffiths2004finding} and usually outperforms the variational
inference approach \ZY{cite ??, and can we create the gibbs sampler
automatically?}.

\begin{figure}[!h]
\footnotesize
\begin{verbatim}
model LDA(alpha, beta, K, vocabSize, N, M) {
  val phi = 
    (0 until K).map(Dirichlet(alpha, vocabSize))
  val theta = 
    (0 until N).map(Dirichet(beta, K))
  val topics = theta.map(theta => 
    (0 until M).map(Categorical(theta)))
  val words = 
    topics.map(z => z.map(Categorical(phi(_))))
}
object LDA extends App {
  /* load hyperparameters and data */
  val m = LDA(alpha, beta, K, vocabSize, N, M)
  m.words.observe(words)
  m.infer()
  print(m.phis)
}
\end{verbatim}
\caption{Latent Dirichlet Allocation in SparkPP}
\label{fig:lda_sparkpp}
\end{figure}


As the corpus size could be as large as several hundred million or billions of
words and the number of parameters could reach the same scale depending on the
hyperparameter settings, it is natural to consider implementing the LDA model
in the distributed system. However the implementation of the LDA model is a
tedious and error-prone process. The GibbsLDA++ is an implementation of
collapsed sampler for LDA on a single machine \cite{gibbslda++} and consists
of 2428 lines of code. The LDA model implemented in MLLib is 826 lines in
length. In SparkPP, the model can be defined in a concise syntax
(\figref{fig:lda_sparkpp}) and inference is taken care of automatically by the
SparkPP compiler. The resulting code is only a few lines long.

\subsection{Gaussian Mixture Model}

\begin{figure}[!h]
\footnotesize
\begin{verbatim}
model GMM(alpha, K, N) {
  val pi = Dirichlet(alpha, K)
  val mu = (0 until K).map(Normal(0, 1))
  val va = (0 until K).map(InvGamma(1, 1))
  val Z = (0 until N).map(_ => Categorical(pi))
  val X = Z.map(z => Normal(mu(z), va(z)))
}
\end{verbatim}
\caption{Gaussian Mixture Model in SparkPP}
\label{fig:gmm_sparkpp}
\end{figure}

Gaussian Mixture Model (GMM) is a common model used in various machine
learning tasks. The data points are assumed to be generated from the mixture
of a number of independent gaussian distributions. Though the
Expectation-Maximization algorithm usually runs much faster than the Bayesian
GMM, the Bayessian GMM captures the uncertainty in the model \ZY{help
robustness?}. GMM in SparkPP (\figref{fig:gmm_sparkpp}) is much simpler than other
implementations.

\subsection{Nonstandard Models}

\begin{figure}[!h]
\footnotesize
\begin{verbatim}
model LDA(alpha, beta, K, vocabSize, N, M) {
  val phi = 
	(0 until N).map((0 until K).map(
		Dirichlet(alpha, vocabSize)))
  val theta = 
    (0 until N).map(Dirichet(beta, K))
  val topics = theta.map(theta => 
    (0 until M).map(Categorical(theta)))
  val words = topics.zip(phi).map{
	case (z, phi) => 
	  z.map(Categorical(phi(_))))}
}
\end{verbatim}
\caption{DCMLDA in SparkPP}
\label{fig:dcmlda_sparkpp}
\end{figure}

In different machine learning tasks, nonstandard models are useful to capture
problem-specific characteristics. In \cite{Doyle2009}, the authors account for
the burstiness in the documents by using per-document topic-word categorical
distributions instead of a global one. The slight change made to the LDA model
requires the inference code to be rewritten while in SparkPP, only a few
adjustments are needed (\figref{fig:dcmlda_sparkpp}).



==> old.tex <==
\subsection{Topic Models}

\begin{figure}[!h] 
	\centering 
	\includegraphics[scale=0.3]{figs/lda.eps}
	\caption{Bayesian Network of Latent Dirichlet Allocation} 
	\label{fig:lda_pgm}
\end{figure}

Topic models are useful statistical models for finding the topics in a corpus.
It has been used to summarize topics in academic papers
\cite{griffiths2004finding}, automatically tag documents, find aspects in
online reviews from Amazon and Yelp \cite{Jo2011}, etc.

Latent Dirichlet Allocation (LDA) is one of the most popular topic model.
\figref{fig:lda_pgm} shows the Bayesian network of the LDA model. The
generative process of the LDA model is as follows. For each topic $k$, a word
distribution $\phi_k$ is chosen from $Dir(\beta, V)$.  $Dir(\beta, V)$ is the
symmetrical Dirichlet distribution of dimension $V - 1$ and parameter $\beta$,
which is a multivariable probability distribution over the space of the space
of all probability mass functions with domain size $V$.  For each document $i$
in the corpus, a topic distribution $\theta_i$ is chosen from $Dir(\alpha, K)$
and for each word $j$ in the document $i$, a topic $z_{ij}$ is chosen from the
topic distribution $\theta_i$ and finally, the word $w_{ij}$ is sampled from
corresponding word distribution $\phi_{z_{ij}}$.  The Bayesian network has the
following joint probability:

{\footnotesize 
\begin{align*} 
	&\mathrm{Pr}(\theta, \phi, z, w) = \\ 
	&\prod_{k=1}^{K}
	\mathrm{Pr}(\phi_k;\beta) \prod_{i=1}^{M} 
	\mathrm{Pr} (\theta_i;\alpha) \prod_{j=1}^{N}
	\mathrm{Pr}(z_{ij}|\theta_i) \mathrm{Pr}(w_{ij}|z_{ij}, \phi) 
\end{align*} 
}

Summarizing the topics in a corpus is one of the main applications of LDA.
Suppose that we have a number of online reviews as input and we want to
summarize two topics from the input. First we can infer the posterior
topic-word distributions $\phi$, which are two Dirichlet distribution with
parameters $\alpha_1$ and $\alpha_2$. Then we pick several words with highest
weights to produce two lists of representative words. Suppose these documents
are online reviews of restaurants and electronic products. If we pick the top
3 words with highest weights in the parameters of the posteriors to represent
the topics, topic 1 may be cooking, taste, service, while topic 2 may be cpu,
performance, price. Thus we find that topic 1 is about restaurants while topic
2 is about electronic products.

Another application of LDA is to add tags to the documents by inferring the
posterior document-topic distributions. In the previous example, an article
can be considered to be related to retaurants if the posterior topic
distribution of the document have higher weight in topic 1 than 2.

Other topic models that are specific to variaous situations are constantly
proposed. The Sentence LDA (SLDA) model assigns only one topic to words in a
sentence to account for the relative positions of words. The Dirichlet
compound multinomial LDA (DCMLDA) model \cite{Doyle2009} uses different
topic-word distributions in each document instead of global ones to account
for the burstiness in a corpus. 


%\small
%\begin{align*}
%	&\mathrm{Pr}(\phi, \theta, z|x) = \\
%	&\frac{
%	\prod_{k=1}^{K} g(\phi^{(k)}; \vec{\alpha}) \prod_{i=1}^{|D|} g(\theta_D;
%	\vec{\beta}) \prod_{j = 1}^{|D_i|} \theta^{(z_{ij})} \phi^{(z_{ij})}_{x_{ij}}
%	}{
%		\int \prod_{k=1}^{K} g(\phi^{(k)}; \vec{\alpha}) \prod_{i=1}^{|D|}
%		g(\theta_D; \vec{\beta}) \prod_{j = 1}^{|D_i|} \theta^{(z_{ij})}
%		\phi^{(z_{ij})}_{x_{ij}} \mathrm{d}z \mathrm{d}\theta \mathrm{d}\phi
%	}
%\end{align*}
%\normalsize

%In Bayesian inference, parameters and data are all treated as random
%variables.  In contrast to frequentist approach \KZ{what exactly is
%frequentist approach} (e.g. support vector machine, k-means clustering) where
%parameters are often treated as unknown fixed constants to be learned,
%parameters in Bayesian inference are model as random variables to capture the
%uncertainty in the parameters. Prior distributions are assigned to parameters
%and the inference task is to calculate the full posterior distribution of the
%parameters given the data. The
%
%
%\figref{fig:lda_pgm} is the Bayesian network of the LDA model.  In a bayesian
%network, nodes are constants and random variables which include parameters and
%data. In the case of LDA, $\alpha$ and $\beta$ are the constant
%hyperparameters that control the shape of the Dirichlet priors for
%document-topic and topic-word distributions. The plate notation is used to
%represent a set of repeated random variables, where the number on the
%lower-right corner is the number of repetitions. $\phi$'s in the LDA are K
%global topic-word distributions, while $\theta$'s are the document-topic
%distributions. $z$'s are latent random variables that represent the topic
%assigments of the observed words $w$ in the corpus.  The edges between nodes
%represent the conditional dependencies and nodes that are not onnected are
%conditionally independent. For example, the word $w$ has incoming edges from
%$z$ and $\phi$'s so the conditional probability of $w$ is $p(w|z,\phi)$. The
%joint distribution represented by the graph is 
%
%{\footnotesize \begin{displaymath} P(\theta, \phi, z, w) = \prod_{k=1}^{K}
%p(\phi_k;\beta) \prod_{i=1}^{M} p(\theta_i;\alpha) \prod_{j=1}^{N}
%p(z_{ij}|\theta_i) p(w_{ij}|z_{ij}, \phi) \end{displaymath} }
%
%
%\begin{figure}[!h] \centering \includegraphics[scale=0.3]{figs/tsm.eps}
%\caption{Bayesian Network of Topic Sentiment Mixture} \label{fig:tsm_pgm}
%\end{figure}
%
%The topic sentiment mixture model \cite{Mei2007} is able to extract both
%topics and sentiments from a corpus (e.g. Amazon reviews). The model is useful
%for generating topic-sentiment summarization and helping predict user behaviours.
%Following the same notation, \figref{fig:tsm_pgm} is the Bayesian network of
%the topic sentiment mixture model for sentiment analysis.  Instead of
%assigning only topics to words in a corpus, TSM model generates words from 4
%types of distributions: a background distribution $\phi_{B}$ for common
%English words, K topic-word distributions $\phi_{i}$ as in LDA, a positive
%sentiment distribution $\phi_{P}$ for words that express positive opinions and
%a negative sentiment distribution $\phi_{N}$ for words that express negative
%opinions. The generative process is as follows: first decide according to a
%constant probability $\lambda$ whether the word comes from background
%distribution. If not, choose a topic according to a document-topic
%distribution $\theta_i$. For each document and each topic, there's a
%categorical distribution $\delta_{ik}$ called sentiment coverage decides
%whether the word is a positve, negative or neutral word, which is indicated by
%the random variable $s_{ij}$.  Then the word is drawn from the corresponding
%word distribution.
%
%After performing inference on the TSM model, we can find an Maximum A
%Posterior (MAP) parameter estimation. With the MAP parameter estimation, the
%TSM model can be used to rank the sentences for the topics using the
%Kullback-Leibler divergence between the language model of the sentences and
%the topic models; or find the sentiment of a sentence by choosing the one that
%has the minimum KL divergence between the language model of the sentence and
%that of the sentiment; or scoring the overall sentiment towards a topic by
%marginalize out the document of the distribution of the sentiment coverages.
%
%Exponential-conjugate Bayesian networks are those that have nodes in
%exponential family and conjugate priors. The exponential family contains
%common distributions like normal distribution, Gamma distribution, Dirichlet
%distribution, categorical distribution and etc. A conjugage prior $P(\theta)$
%to a likelihood function $P(x|\theta)$ is one whose the posterior distribution
%$P(\theta|X)$ is in the same family as the prior distribution. For example, if
%a Dirichlet prior is for a categorical distribution, the posterior is still a
%Dirichlet distribution with different parameters. It's a restricted yet useful
%subset of Bayesian networks, which is used in many applications. More
%importantly, these Bayesian networks can be dealt with by the automated
%inference tools efficiently using variational inference or Gibbs sampling with
%little user tuning. Strictly speaking, the LDA model and the TSM model are not
%in exponential family because they have mixtures of exponential distributions.
%But this problem can be solved by introducing latent variables (e.g. topics
%$z$ in LDA, $b$, $s$, $z$ in TSM). The resulting models are still able to be
%handled by the automated inference tools.
%
%\KZ{can handle arbitrary models and why mllib cannot easily handle them?  put
%pgms of different models (not limited to exponential-conjugate models), need
%applications to justify the need of a PL} 
%
%\ERIC{subsection 1. pgm and models; what are input and queries; subsection 2.
%how to use inferSpark;
%BASELINE solution}
%
%\KZ{move the following to this section}
%For example, the Topic Sentiment Mixture model \cite{Mei2007}, which is used
%to generate topic-sentiment summarization of a corpus (e.g. online reviews)
%and help predict user behaviour, is a Bayesian network that encodes
%dependencies between the latent sentiment and topic variables and the data.
%The topic-sentiment analysis task is done by performing inference on the
%Bayesian network, or in other word calculating the posterior distribution of
%the latent variables given the corpus.


%\subsection{InferSpark Syntax}

%An InferSpark model definition has similar syntax with normal Scala
%class/object definition. It can reside in the same file as other scala code.
%\figref{fig:lda_model} is the model definition of LDA. The model definition
%starts with the ``@model'' annotation, followed by a class definition. The
%class parameters (K, V, alpha, beta) are treated as constants in the model,
%which will be determined at runtime but prior to the execution. The only
%allowed definitions inside the classbody are the definitions of random
%variables prefixed with ``val''.  Ranges represent the plates in Bayesian
%networks. For example, line 3 in the LDA model definition defines a plate of
%Dirichlet variables with size K. Line 4 uses a special kind of range ``?'' in
%InferSpark, which means the size of the plate is unknown at the time of model
%definition but will be inferred from the observed variables. As in line 5 and
%6, random variables mapped from previous declared random variables will share
%the plates. When any one of ``theta'' , ``z'' and ``x'' is declared observed
%by providing an RDD of data, the size of ``?'' in line 4 will be calculated
%automatically. ``?'' syntax also naturally handles the situation where each
%documents have different lengths.  In line 6, Categorical(phi(z)) defines a
%mixture of categorical distributions of phi whose mixture probability is
%$\mathrm{Pr}(z)$.



%\begin{figure}[h]
%\begin{lstlisting}
%def infer(): LDA {
%	val xdata: RDD[Array[Long]] = /* load data */
%	val lda = new LDA(K, V, alpha, beta)
%	lda.doc.x.observe(xdata)
%	lda.infer(nIterations)
%	lda.phi.getResult().map{
%	case (vid, result) =>
%		val words = (0 until V).map{word =>
%			(word, result.pseudoCount(word))
%		}.sortBy(_._2)(math.Ordering.Double.reverse)
%		(vid - lda.phi.baseId, words.take(10))
%	}.collect().foreach(println)
%	lda
%}
%\end{lstlisting}
%\label{fig:lda_inference}
%\caption{Calling Inference API}
%\end{figure}

%\begin{figure}[h]
%\begin{lstlisting}
%def predict(lda: LDA) {
%	/* load data */
%	val xpred_data: RDD[Array[Long]] = /* ... */
%	val ldapred = new LDA(K, V, alpha, beta)
%	ldapred.phi.observe(lda.phi.getResult())
%	ldapred.theta.observe(lda.theta.getResult()) 
%	ldapred.x.inferLengthFrom(xpred_data)
%	ldapred.infer(nIterations)
%	val perplexity = 
%	ldapred.x.makeJoinable(xpred_data).innerJoin(ldapred.x.getResult()).map{ 
%	(_, word, result) => 
%		-Math.log(result.probability(word))
%	}.map(_._2).reduce(_ + _) / ldapred.x.count
%	println("perplexity = " + perplexity)
%}
%\end{lstlisting}
%\label{fig:lda_prediction}
%\caption{Prediction using Inference Result}
%\end{figure}
%
%In some cases, it would be useful to set the size of plate without observe
%the variables (e.g. making predictions using the inference result).
%Line 7 of \figref{fig:lda_prediction} shows how to achieve this. When
%``inferLengthFrom'' is called, the sizes of plates are calculated as if
%``observe'' is called, but the random variable is still unobserved.

%\begin{figure}[!h]
%\footnotesize
%\centering
%\begin{verbatim}
%model TSM(alpha: Double, lambda: Double, 
%          phi_B: Array[Double], beta: Double, 
%          beta_P: Double, beta_N: Double,
%          V: Long, K: Long, D: Long, N: Long) {
%  val phi = (0 until K).map(_ => 
%    Dirichlet(beta, V))
%  val phi_P = Dirichlet(beta_P, V)
%  val phi_N = Dirichlet(beta_N, V)
%  val theta =  (0 until D).map(_ =>
%      Dirichlet(alpha, K))
%  val delta = (0 until D).map(_ =>
%      (0 until K).map(Dirichlet(1, 3)))
%  val b = (0 until D).map(_ =>
%      (0 until N).map(_ => Bernoulli(lambda)))
%  val z = theta.map{ theta =>
%    (0 until N).map(_ => Categorical(theta))}
%  val s = delta.map{ delta =>
%    (0 until N).map(_ => Categorical(delta))}
%  val w = b.zip(z).zip(s).map{case ((b,z),s) =>
%    (0 until N).map(j => Categorical(
%      if (b(j)) phi_B
%      else if (s(j) == 0) phi_P
%      else if (s(j) == 1) phi_N
%      else phi(z(j))))}
%}
%\end{verbatim}
%\caption{Topic Sentiment Mixture in InferSpark}
%\label{fig:TSM_pp}
%\end{figure}
%
%LDA is a well-studied with wide application. Hence, a lot of machine learning
%libraries including MLLib implement collapsed Gibbs Sampler, an efficient
%inference algorithm, for the LDA model. When it comes to the customized models
%like the Topic Sentiment Mixture model (see \figref{fig:tsm_pgm}) for
%sentiment analysis, there is no off-the-shelf libraries to use. The user has
%to derive the formula and implement the algorithm by themselves. But with
%InferSpark, the user simply has to write a simple model definition and call
%the APIs using a dozens of lines.
%
%
%\begin{figure}[!h]
%\begin{verbatim}
%object Main extends Apps {
%  /* load parameters */
%  val w = sc.textFile("hdfs://localhost/corpus.txt")
%  val m = TSM(...)
%  m.w.observe(w)
%  m.infer(qualityEvaluator=f, initialIter=10, iter=100)
%  val posterior_phi_P = m.phi_P.posterior
%  /* ... */
%}
%\end{verbatim}
%\caption{Calling InferSpark API on the TSM model}
%\label{fig:TSM_API}
%\end{figure}
%
%In the scala program, the user can create an instance of a model in the
%same way as creating an instance of a class. Each random variable defined in
%the model is a field of the model object. The user can specify the observed data by
%invoking the obesrve method of the corresponding random variable. In the infer
%method of the model object, the ruse can specify parameters to the inference
%engine or rely on the default behaviour. If the user provides a
%quality evaluator and there is more than one available algorithm, both
%algorithm will be run for some initial iterations. Then the quality evaluator
%will be called to evaluate the qualilty of inference and the inference engine
%will heuristically choose the better one to run to the end.
%
%After the inference is finished, the user could launch 3 types of
%queries about the results: expectation query $E[g(\theta)|X]$, posterior
%parameter query and MAP query. The compiler will inspect the queries in user's
%scala program to determine what algorithms are applicable to the inference
%tasks.


==> old_intro.tex <==
\section{Introduction}
\label{sec:intro}

\subsection{Motivation}
\KZ{Our problem is expoential-conjugate bayesian network and
why it's an important and general domain of problems.}

% wide application
Bayesian inference is an important technique to express hypothesis and reason
about observed data. Bayesian approach assigns priors to the parameters in the
models and captures the uncertainty of the parameters by calculating the
posterior distributions instead of treating parameters as fixed unknown
constants. Bayesian networks are a flexible and power tool to specify the
dependencies of random variables and encode probability distributions.
Bayesian networks have been used in a wide range of scientific research. 

Exponential-conjugate Bayesian networks are those that have nodes in
exponential family and conjugate priors. It's a restricted yet useful subset
of Bayesian networks, which is used in various areas like topic modelling,
sentiment analysis and etc.\cite{Titov2008a, Titov2008b, Jo2011} For example,
the Topic Sentiment Mixture model \cite{Mei2007} extracts topics and
sentiments from blogs. Different from the standard LDA model, it incorporates
latent variables to represent positive/negative setiments in each topic. The
model is useful to generate topic-sentiment summarization of a corpus and help
predict user behaviour.

\begin{figure}[!h]
	\epsfig{file=figs/tsm,scale=0.3}	
	\caption{Topic Sentiment Mixture Model}
	\label{fig:TSM_model}
\end{figure}

\KZ{Give detailed applications and is possible their graphical models in pics.}
\KZ{Why programming language (and specifically PP) is the right 
approach for solve these bayesian network inference problems.}

To perform Bayesian inference, the user could use an off-the-shelf
implementation from an existing machine learning library but his choice is
constrained to the models that the library support, which usually are standard
ones like the latent Dirichlet allocation model. When the application needs a
non-standard model to capture the characteristics in the problem, the user,
however, have no choice but to develop his own code. Developing inference code
requires extensive knowledge in both Bayesian inference and programming
techniques. Moreover, model definition, inference algorithm and unrelated code
are all mixed up in the resulting code, making it hard to debug and resaon
about.

Probabilistic proramming languages are designed to cope with the problem.  User
only needs to specify the model in a concise syntax and the inference is
handled automatically by the compiler and the runtime system for
exponential-conjugate and other certain kinds of Bayesian networks.  The
inference code generated by the compiler could be as efficient as that
carefully optimized by the user.

\KZ{Why there is a need to extend PP to distributed/parallel computing.}
% large data set
\KZ{Stick to the speech/topic examples. You need
a couple of driving examples and keep using them.}

When applying Bayesian inference, the huge data size often overwhelms the
capacity of a single machine. For example, when the TSM model extracts users'
positive/negative opinion from hundreds of millions Amazon reviews, the data
could be too large to fit into the memory of a single machine and even if it
does, training will take days or weeks. To perform the inference task
efficiently, the user has to resort to a distributed and parallel solution, in
which case the training may only takes hours. But it is hard and
time-consuming to write and tune inference code for large scale data even if
the user uses popular distributed computing frameworks \cite{Cai2014}. The
problem applys to other models in various applications.

\KZ{Why existing PP cannot be easily extended to distributed framework
and how we are diff from them.}
%% Existing pp
It is useful to have a probabilistic programming language that supports
flexible user-defined models and that is able to perform distributed and
parallel inference automatically. However, existing probabilistic programming
languages (e.g. Figaro \cite{pfeffer2009figaro}, Infer .NET \cite{InferNET14},
FACTORIE \cite{McCallum2009}) have put more emphasis on the expressibility and
inference algorithms. They are designed for a multi-threaded or
single-threaded machine and hard to be ported to distributed computing
frameworks. For example, the Figaro model objects are mutable and caches
current values while Spark RDD stores immutable objects. It is not possible to
overcome the problem without make significant amount of changes to the Figaro
library.

\subsection{Our solution}

Our solution is to design a probabilistic programming language embedded in
scala and base its inference engine on Spark, a high-performance distributed
data processing framework.

We currently only focus on exponential-conjugate models so that the posterior
has known forms and inference can be handled by efficient algorithms
automatically. Variational message passing and Gibbs sampling are two
algorithms that can be applied to these models without any user derivation.

\subsection{Contributions}

\begin{itemize}
	\item We design a probabilistic programming language embedded in scala
		that can be used to concisely represent bayesian networks.
	\item We implement efficient inference algorithms on Spark to enable
		automatic inference on large-scale data.
\end{itemize}



==> old_motivate.tex <==
\section{A Motivating Example}
\label{sec:motivate}

TrueSkill \cite{ralf2007trueskill} is a Bayesian skill rating model developed by Microsoft Research. We consider a simplified model.

Suppose we have N players, each pair of them played a game. We model the skill of each player as random draws from a gaussian prior. The result of a game depends on which player has performed better, which is a random variable draw from a gaussian distribution with the skill as its mean. The factor graph of the model is shown in \figref{fig:trueskill_factors}.

\ZY{insert the trueskill factor graph here}
\begin{figure}[h]
\centering
\epsfig{file=trueskill_factor_graph,scale=0.5}
\caption{True skill factor graph}
\label{fig:trueskill_factors}
\end{figure}

Given the game results, we want to infer the skills of each player. We only need
to encode the model in PP which is straight-forward (\figref{fig:trueskill_code}) and
obtain the inference results by calling API.

\begin{figure}[h]
\centering
\begin{verbatim}
model Skill(n: Int) {
  val skill ~ pp.Array.
    tabulate(gaussian(100, 10))
  val perf ~ skill.map(
    s => gaussian(s, 20))
  val results = perf.zip(perf).map{ 
    (p1, p2) => p1 > p2 }
}

object Skill extends App {
  /* data loading */
  val model = new Skill(n)
  model.observe_results(results)
  model.infer()
  model.skill.foreach{
    s => println(s.mean)
  }
}
\end{verbatim}
\vspace{-15pt}
\caption{True skill code in PP}
\vspace{-5pt}
\label{fig:trueskill_code}
\end{figure}

The first line in model definition defines an array of the skills of n players to be independently drawn from the gaussian prior. The next line draws the performance of each player from a gaussian distribution with mean of corresponding skills by perform a mapping operation. The last line results are deterministically computed by comparing the performances of each pair of players. Half of the results are duplicates but we just omit the details for simplicity.

The object Skill defines the entry function of the program. It loads the data, creates a new instance of the Skill model and supplies the observation by calling observe\_results method of it. The inference algorithm is executed by calling infer method and finally the means of each players' posterior skills are queried by referencing the mean member of the skill variables.

Since MLlib is not applicable to the customized model, we would be forced to write hundreds of lines of code to implement the model directly in Spark without PP. We need to create classes from scratch to represent the factors of the model and carefully implement an inference algorithm. Debugging could be another challenge in distributed applications. It would be hard for domain experts who do not have significant knowledge in Bayesian inference or programming techniques to implement these customized models. Existing PP also would not work when the data gets too large to fit in the main memory. 

With a probabilistic programming language built on Spark, we can write code as simple as the the above example while leveraging the scalability enabled by Spark. The ease of developing probabilistic models means more attention could be paid to the design and the tuning of the model rather than coding.



==> pplang.tex <==
\section{InferSpark Language and API}
\label{sec:pplang}

\begin{figure}[!h]
\footnotesize
\centering
\begin{verbatim}
model TSM(alpha: Double, lambda: Double, 
          phi_B: Array[Double], beta: Double, 
          beta_P: Double, beta_N: Double,
          V: Long, K: Long, D: Long, N: Long) {
  val phi = (0 until K).map(_ => 
    Dirichlet(beta, V))
  val phi_P = Dirichlet(beta_P, V)
  val phi_N = Dirichlet(beta_N, V)
  val theta =  (0 until D).map(_ =>
      Dirichlet(alpha, K))
  val delta = (0 until D).map(_ =>
      (0 until K).map(Dirichlet(1, 3)))
  val b = (0 until D).map(_ =>
      (0 until N).map(_ => Bernoulli(lambda)))
  val z = theta.map{ theta =>
    (0 until N).map(_ => Categorical(theta))}
  val s = delta.map{ delta =>
    (0 until N).map(_ => Categorical(delta))}
  val w = b.zip(z).zip(s).map{case ((b,z),s) =>
    (0 until N).map(j => Categorical(
      if (b(j)) phi_B
      else if (s(j) == 0) phi_P
      else if (s(j) == 1) phi_N
      else phi(z(j))))}
}
\end{verbatim}
\caption{Topic Sentiment Mixture in InferSpark}
\label{fig:TSM_pp}
\end{figure}

LDA is a well-studied with wide application. Hence, a lot of machine learning
libraries including MLLib implement collapsed Gibbs Sampler, an efficient
inference algorithm, for the LDA model. When it comes to the customized models
like the Topic Sentiment Mixture model (see \figref{fig:tsm_pgm}) for
sentiment analysis, there is no off-the-shelf libraries to use. The user has
to derive the formula and implement the algorithm by themselves. But with
InferSpark, the user simply has to write a simple model definition and call
the APIs using a dozens of lines.

An InferSpark model definition has similar syntax with normal Scala
class/object definition. The model definition starts with the ``model''
keyword, which is followed by an identifier and a model parameter list. The
parameters are constants in the model. Definition of random variables prefixed
with ``val'' and pure functions prefixed with ``def'' are allowed. The random
variables are either primitive random variables or collections of random
variables. For example, phi\_P in the TSM model is a primitive random variable
of Dirichlet distribution with type Vector[Double]; phi is a collection of
primitive random variables of Dirichlet distribution with type
Vector[Vector[Double]]; w is a collection of a collection of random variables
of Categorical distribution with type Vector[Vector[Int]]. For primitive
types, the pure functions (e.g. log, exp) can be applied to them if the type
matches the parameter type. For collection types, the common collection
methods like map/reduce can be used but functions that accept a concrete
collection type cannot be applied since the types of collection could become
RDD during inference.

\begin{figure}[!h]
\begin{verbatim}
object Main extends Apps {
  /* load parameters */
  val w = sc.textFile("hdfs://localhost/corpus.txt")
  val m = TSM(...)
  m.w.observe(w)
  m.infer(qualityEvaluator=f, initialIter=10, iter=100)
  val posterior_phi_P = m.phi_P.posterior
  /* ... */
}
\end{verbatim}
\caption{Calling InferSpark API on the TSM model}
\label{fig:TSM_API}
\end{figure}

In the scala program, the user can create an instance of a model in the
same way as creating an instance of a class. Each random variable defined in
the model is a field of the model object. The user can specify the observed data by
invoking the obesrve method of the corresponding random variable. In the infer
method of the model object, the ruse can specify parameters to the inference
engine or rely on the default behaviour. If the user provides a
quality evaluator and there is more than one available algorithm, both
algorithm will be run for some initial iterations. Then the quality evaluator
will be called to evaluate the qualilty of inference and the inference engine
will heuristically choose the better one to run to the end.

After the inference is finished, the user could launch 3 types of
queries about the results: expectation query $E[g(\theta)|X]$, posterior
parameter query and MAP query. The compiler will inspect the queries in user's
scala program to determine what algorithms are applicable to the inference
tasks.




==> runtime.tex <==
\subsection{Runtime system}
\label{sec:runtime}

\begin{itemize}
\item Data partition

\item Operations in inference algorithms.
\end{itemize}

\cut{%%%%%%%%%%%
Data in Spark are represented as resilient distributed datasets \cite{Zaharia:2012:RDD:2228298.2228301} and Spark provides the GraphX that supports parallel graph computations. For large models, the number of nodes in the factor graph could be huge so it is natural to represent the factor graphs using GraphX. Moreover, many inference algorithms can be expressed as message passing algorithms \cite{koller2009probabilistic} which can be efficiently implemented in GraphX. We will explore the efficient implementation of these inference algorithms and use them as the default inference algorithm.

Alternatively, we can perform inference by drawing samples from the posterior distribution using the Metropolis-Hastings algorithm adapted from \cite{wingate2011lightweight}.
First, all variables are initialized with some value that satisfy the given observations of variables. 
In each step, a new random value is proposed for a randomly selected random variable based on its current value and parameters. 
The whole execution trace is adjusted accordingly so that the execution trace is consistent with the update. 
Whether the proposed update is accepted or rejected depends an acceptance rate computed using the following formula:
\begin{equation*}
	\alpha_{X \rightarrow X'} = \min\{{1, \frac{P(X')Q(X'\rightarrow X)}{P(X)Q(X \rightarrow X')}\}}
\end{equation*}
where $X$ and $X'$ are the old and new execution trace, $P(\cdot)$ is the forward probability of the execution trace 
and $Q(X \rightarrow X')$ is the probability that a proposal is made to update from $X$ to $X'$.

It essentially constructs a Markov chain in the space of all valid execution traces. 
The samples drawn from the chain will converge to the posterior distribution determined by
the model and the observed value for by accepting the proposed update with probability $\alpha_{X \rightarrow X'}$.
Thus detailed balance condition is satisfied, which ensures the chain will converge to the distribution
with probability function $P(\cdot)$. Note that we only need to use the forward probability of the execution trace since
any trace that does not satisfy the observation is invalid, i.e. not in the space of the Markov
chain. The forward probability is essentially the unnormalized posterior probability. The formula
is unchanged by dividing the numerator and denominator with the same normalizing constant.

Forward probability can be easily calculated by the product of the probabilities of value of all the random
variables. For large models, it is very costly to compute but with Spark we can implement it in terms of
efficient MapReduce operations.

In addition to the built-in algorithms, user can define customized algorithms by implementing the abstract algorithm interface in the runtime system. By switching to customized algorithms, inference on specific models can be made more efficient and useful. For example, user can implement the parallel Gibbs sampling \cite{wang2009plda} for Latent Dirichlet Allocation \cite{blei2003latent} using the Spark MapReduce operation. The runtime saves users' labor by providing a ready-to-use class definition of the model and users only need to implement the infer method. The implementation of infer involves no more than a few lines of map reduce operations on the factors.

}%%%%%%%%%%%%%%%


==> syntax.tex <==
\section{Syntax \& Semantics}
\label{sec:syntax_semantics}

\begin{figure}[!h]
\small
	\begin{tabular}{lrl}
		ModelDef & ::= & `model' id `\{' ModelStmts `\}' \\
		ModelStmts & ::= & ModelStmt [[semi] ModelStmts] \\
		ModelStmt & ::= & `val' PatDef \\
				  & $|$ & `def' FuncDef \\
		\multicolumn{3}{c}{...} \\
		SimpleExpr & ::= & Dist ArgumentExprs \\
				   & $|$ & ScalaSimpleExpr
	\end{tabular}
\caption{SparkPP Syntax}
\label{fig:sparkpp_syntax}
\end{figure}

SparkPP's syntax of model definition is an extension of the functional subset
of the syntax of scala. ... 

\begin{figure}[!h]
\small
\begin{tabular}{lrlr}
	$m$ & ::= & $c$ & (constants) \\
	  & $|$ & $X$ & (variables) \\
	  & $|$ & $dist$($\vec{m}$) & (primitive distributions) \\
	  & $|$ & $m_1$($\vec{m_2}$) & (function application) \\
	  & $|$ & let $X$ = $m_1$ [in $m_2$] & (bindings) \\
	  & $|$ & $\lambda$ $x$. ScalaExpr & (function def.) \\
	$\vec{m}$ & ::= & $\varepsilon$ & (empty argument list) \\
			& $|$ & $m_1$, $\vec{m_2}$ & \\

\end{tabular}
\caption{Core Syntax}
\label{fig:core_syntax}
\end{figure}

The semantics of the model definition is the probability distribution
represented by the generative process in the model definition. The
distribution can be uniquely determined by its probability mass function (pmf)
since all types in scala have a finite domain (including integer and floating
point numbers).

To simplify the definition of the formal semantics of SparkPP models, we
define a simplified core syntax \figref{fig:core_syntax}. A SparkPP model can be
easily transformed into the core syntax and share the same semantics.


\begin{figure}[!h]
\tiny

\inference[1)]{{\begin{array}{l}
	\texttt{let } Y' \texttt{ be a fresh variable} \\ 
	\var(P') = \var(P) \cup \{Y'\} \\
	\forall v \in \dom(\var(P)), y' \in \dom(Y'), \\
	\qquad P'(\var(P) = v, Y' = y') = \left\{{
				\begin{array}{lr}
					P(\var(P) = v) & (y' = c) \\
					0 & (y' \neq c)
				\end{array}}\right.%}
\end{array}}}
{(P, E, Y, c) => (P', E, Y')}

\inference[2)]{{\begin{array}{l}
	Y' = \left\{{\begin{array}{lr}
		X & (X \in \var(P)) \\
		E[X] & (X \in E)
	\end{array}}\right.%}
\end{array}}}
{(P, E, Y, X) => (P, E, Y')}

\inference[3)]{{\begin{array}{l}
	(P, E, Y, \vec{m}) => (P', \_, \_) \\
	\texttt{let } Y' \texttt{ be a fresh variable} \\ 
	\var(P'') = \var(P') \cup \{Y'\} \\
	\forall v \in \dom(\var(P')), y' \in \dom(Y'), P''(\var(P') = v, Y' = y') = \\
	\qquad P_{dist}(Y' = y'; Eval(\vec{m} | Var(P')))P'(\var(P') = v)
\end{array}}}
{(P, E, Y, dist(\vec{m})) => (p'', E, Y')}

\inference[4)]{{\begin{array}{l}
	(P, E, Y, \vec{m}) => (P', \_, \_) \\
	\texttt{let } Y' \texttt{ be a fresh variable} \\ 
	\var(P'') = \var(P') \cup \{Y'\} \\
	\forall v \in \dom(\var(P')), y' \in \dom(Y'), \\
	\qquad f = func(Eval(\vec{m} | \var(P') = v)) \\
	\qquad P''(\var(P') = v, Y' = y') = \left\{{
		\begin{array}{lr}
			P'(\var(P') = v) & (y' = f) \\
			0 & (y' \neq f)
		\end{array}}\right.%}
\end{array}}}
{(P, E, Y, m_1(\vec{m_2})) => (P'', E, Y')}
	
\inference[5)]{{\begin{array}{l}
	(P, E, Y, m_1) => (P', \_, Y') \\
	\texttt{if } Y' \texttt{ is an R.V.} \\
	{\begin{array}{l}
		\quad \texttt{create a fresh variable named } X \\
		\quad \texttt{let } V = \var(P'') - \{Y'\}
		\quad \var(P'') = \var(P') \cup \{X\} \\
		\quad \forall v \in \dom(V), y' \in dom(Y'), x \in \dom(X), \\
		\qquad P''(V = v, Y' = y', X = x) = \left\{{
			\begin{array}{lr}
				P'(V = v, Y = y) & (x = y) \\
				0 & (x \neq y)
			\end{array}}\right. \\
		\quad E' = E
	\end{array}} \\
	\texttt{elif } Y' \texttt{ is a function} \\
	{\begin{array}{l}
		\quad P'' = P'
		\quad E' = E \cup {X : Y'}
	\end{array}}
\end{array}}}
{(P, E, Y, \texttt{let } X = m_1) => (P'', E', U)}

\inference[6)]{{\begin{array}{l}
	(P, E, Y, \texttt{let } x = m_1 => (P', E', U) \\
	(P', E', U, m_2) => (P'', E'', Y')
\end{array}}}
{(P, E, Y, \texttt{let } X = m_1 \texttt{ in } m_2) => (P'', E'', Y')}

\inference[7)]{}
{(P, E, Y, \lambda\texttt{ }x.\texttt{ScalaExpr}) => (P, E, \lambda\texttt{ }x.\texttt{ScalaExpr})}

\inference[8)]{}{(P, E, Y, \varepsilon) => (P, E, U)}

\inference[9)]{{\begin{array}{l}
	(P, E, Y, m_1) => (P', \_, \_) \\
	(P', E, U, \vec{m_2}) => (P'', \_, \_)
\end{array}}}
{(P, E, Y, m_1, \vec{m_2}) => (P'', E, U)}

\caption[SparkPP Semantics]{SparkPP Semantics. \\
\texttt{$P$ $\in$ $\Omega$ $\rightarrow$ $[0, 1]$, the space of all possible p.m.f over a
finite set of random variables. $E[x]$ is the function binded to variable $x$.
$Eval(\vec{m} | \var(\vec{m}))$ is the evaluation result of the argument list
$\vec{m}$ given the assignment of $\var(\vec{m})$ under the normal scala
semantics.}}
\label{fig:semantics}
\end{figure}

The semantics of a model definition is the probability mass function of the
distribution represented by the generative process. The process is represented
by a triple $(P, E, Y)$ of the probability mass function so far and the
function bindings and the value that the model evaluates to (r.v. or function).
$(P, E, Y, prog)$ $\Rightarrow$ $(P', E', Y')$ means that $prog$ transforms
$(P, E, Y)$ into $(P', E', Y')$. Then we can define the semantics of a model
$m$ to be P where $(P_0, \Phi, U, m) \Rightarrow (P, E, Y)$ for some $E$ and
$Y$. $\var(P_0) = \{U\}$ where $U$ is different from all possible variables and
has a domain size of 1.


\begin{itemize}
\item Typing rules. 

\item Query semantics: given a joint distribution
and observed data,  return expectation, sample and MAP.

\end{itemize}


==> vmp.tex <==
\section{Variational Message Passing}

Let $\Theta$ be the set of hidden variables and $X$ be the observed variables.
parametric family of distributions. We use capital letters $P$, $Q$ to
represent distributions, and corresponding small letters $p$, $q$ to denote
its probabilistic density function or probability mass function.
Variational inference approximates the posterior distribution
$P_{\Theta|X}$ with a distrbution $Q_{\Theta}$ from a
A simple choice of the
approximating
family is,
\begin{equation*}
	q(\Theta) = \prod_{\theta \in \Theta} q(\theta)
\end{equation*}
, the fully factorized family over the parameters. This choice assumes that
all hidden variables are independent in the approximate distribution. Since
the independence assumption may not be true in the posterior distribution, the
algorithm may not be able to find the exact posterior distribution. The
algorithm iteratively minimizes the Kullback-Leibler divergence
$\mathrm{KL}(Q||P)$ between the approximate distribution and
the true distribution so that the approximate distribution is as close as
possible to the true posterior. Although the KL divergence cannot be computed
without knowing the true posterior, it is not necessary to
directly optimize the KL divergence. Instead, the algorithm maxmizes the
evidence lower bound (ELBO) 
\begin{equation}
	\label{eqn:ELBO}
	\mathcal{L}(Q) = E_Q[\ln p(\Theta, X) - \ln q(\Theta)] 
\end{equation} 
, maximizing which is equivalent to minimizing the KL divergence. ELBO only
involves the expectation of the log likelihoods in terms of the approximate
distribution $Q$ and it is straight forward to calculate. 

Separating out terms related to one of the hidden variables $\theta \in
\Theta$ and let $F_{(\cdot)}$ be the parent of the variable and
$\mathrm{C}_{(\cdot)}$ be the set of children of the variable, the ELBO can be
rewritten as
\begin{align*}
	&\mathcal{L}(Q) = -\mathrm{KL}(Q_\theta || \tilde{P}_\theta) +
	\mathrm{Const}(\theta) \numberthis \label{eqn:ELBO_one_term}
\end{align*}
, where $\mathrm{Const}(\theta)$ is a constant with respect to $\theta$ and $\tilde{P_\theta}$ is defined as
\begin{align*}
	&\ln\tilde{p}(\theta) = E_{Q_{\Theta \backslash
	\theta}}[\ln p(\theta|\mathrm{F}_\theta) + \sum_{\phi \in
	\mathrm{C}_\theta }p(\phi|\mathrm{F}_\phi)] + Z
\end{align*}
$Z$ is a normalizing constant. The KL divergence is always non-negative. It
equals to zero if and only if the two distributions are the same. Therefore,
setting $Q_\theta$ to $\tilde{P}_\theta$ maximizes the ELBO with regard to
$\theta$.  Since the model is in exponential family and have conjugate priors,
all terms in $\ln \tilde{p}(\theta)$ has the same form of the dot product of
parameters and sufficient statistics except the normalizing constant.
Therefore, the ELBO is maximized by letting $\ln q(\theta)$ have the same form
as $p(\theta|\mathrm{F}_\theta)$ and setting the parameters to those of
$\tilde{P_\theta}$.  In the coin flipping case, if the probability of head has
$\mathrm{Beta}(\alpha, \beta)$ prior,
\begin{align*}
\ln\tilde{p}(\phi) &= [\alpha - 1 \quad \beta - 1] 
	\begin{bmatrix} \ln \phi \\ \ln(1-\phi) \end{bmatrix}  \\
	&+ [H \quad N-H]  \begin{bmatrix} \ln \phi \\ \ln(1-\phi) \end{bmatrix} + Z
\end{align*}
The ELBO is maximized when the $Q$ is set to $\mathrm{Beta}(\alpha + H,
\beta + N - H)$. Note in the one coin model, $Q$ is exactly the true
posterior in \eqnref{eqn:coin_posterior} because the independence assumption
naturally holds for a univariate distribution.

\begin{figure}[h]
	\includegraphics[scale=0.5]{figs/two_coins_latent.eps}
	\label{fig:two_coins_latent}
	\caption{Introducing additional hidden variables to mixture model}
\end{figure}

Mixture models (e.g. flipping two coins) are no longer in Exponential conjugate
family. To apply the variational algorithm, the trick is to introduce
additional hidden variables. For example, we can add the choice of the coins
(i.e. $z_i$ in \figref{fig:two_coins_latent}) for each of the outcomes. Let
$z_{ik} = 1$ if $z_i = k$, $z_{ik} = 0$ otherwise, and $x_{i} = 1$ if $x_i$ is
head, $x_{i} = 0$ if $x_i$ is tail, the log likelihood of
$x_i$ is 
\begin{align*}
	\ln p(x_i|\phi_1, \phi_2, z_i) = \sum_{k=1}^2 z_{ik} [x_{i} \quad 1-x_{i}]
\begin{bmatrix} \ln \phi_k \\ \ln (1-\phi_k) \end{bmatrix}
\end{align*}
The log likehood has the same forms as the prior $\ln f(\phi_k; \alpha, \beta)$.
Hence the model is conjugate.

The updates to the parameters of approximate distributions $Q$
are the aggregation of terms that either only depends on the parent or depends
on one child and the other parents of it. The terms in the updates can be
computed locally at the neighbours of the updated random variable.  For
example, the update of $z_i$'s parameters in the
two coins model is
\begin{equation}
	E[\ln \pi] + E[\ln p(x|\phi)]
\end{equation}
The first term can be computed locally at $\pi$ and the second term can be
computed locally at $x_i$ given $\phi_1$ and $\phi_2$.  The VMP algorithm
defines the terms as messages to be sent along both directions of edges in the
Bayesian network. In each step, one of the vertecies is chosen to pull
messages from its neighbours and update itself by aggregating the messages.
If a message is from the child and also depends on co-parents, the child will
pull messages from the co-parent as well. 

